Mining Generalized Patterns from Large Databases using Ontologies

Formal Concept Analysis (FCA) is a mathematical theory based on the formalization of the notions of concept and concept hierarchies. It has been successfully applied to several Computer Science fields such as data mining,software engineering, and knowledge engineering, and in many domains like medicine, psychology, linguistics and ecology. For instance, it has been exploited for the design, mapping and refinement of ontologies. In this paper, we show how FCA can benefit from a given domain ontology by analyzing the impact of a taxonomy (on objects and/or attributes) on the resulting concept lattice. We willmainly concentrate on the usage of a taxonomy to extract generalized patterns (i.e., knowledge generated from data when elements of a given domain ontology are used) in the form of concepts and rules, and improve navigation through these patterns. To that end, we analyze three generalization cases and show their impact on the size of the generalized pattern set. Different scenarios of simultaneous generalizations on both objects and attributes are also discussed

==> Introduction.tex <==
%\section{Introduction}\label{S:intro}
Formal Concept Analysis (FCA) is a formalism for knowledge
representation which is based on the formalization of ``concepts''
and ``concept hierarchies'' \cite{GW99}. In traditional philosophy,
a concept is considered to be determined by its extent and its
intent. The extent contains all entities (e.g., objects,
individuals) belonging to the concept while the intent includes all
properties common to all entities in the extent. The concept
hierarchy states that ``a concept is more general if it contains
more entities'' and is also called a specialization-relation on
concepts. FCA lies on the mathematical notions of  binary relations,
Galois connections and ordered structures and has its roots in the
philosophy. It provides methods to extract and display knowledge
from databases and has many applications in knowledge representation
and management, data mining, and machine learning.

In philosophy, ontology is the study of the categories of things that exist or
may exist in a specific domain. In computer science, it is an explicit conceptualization of a given domain %such as air traveling
in the form of concepts and their relations (roles), as well as
concept instances that are linked by relations instantiating generic
roles. Roles are usually directed so that a given role maps the
instances of a source concept
%(e.g., a passenger)
to those of a target one. %(e.g., a flight).
Ontology design and utilization are presently gaining an increasing
interest with the emergence of the Semantic Web
\cite{berners-semanticweb01}, and standardization efforts are
progressing in the field of ontological languages such as OWL. Many
studies were concerned with ontology construction, mapping and
integration \cite{kalfoglou05,Noy04}.

In ontology, a concept can be understood as its FCA-intent
(attributes), and the FCA-entities (objects) as instantiations of
concepts. One particular relation between concepts represents the
{\em is-a} hierarchy. This corresponds to the
specialization-relation in FCA, and provides a taxonomy on the
attributes of the domain of interest. The primary goal of an
ontology is to model the concepts and their relations on a domain of
interest, whilst FCA aims to discover concepts from a given data
set. Within FCA, an interactive method for knowledge acquisition
called ``attribute exploration'' has been developed to discover and
express knowledge from a domain of interest with the help of a
domain expert \cite{Gb87,Ganter99attributeexploration,GW86}. This
method has been widely used for ontology engineering and refinement
(see Section~\ref{S:relatedwork}).

FCA and Ontology both use ordered structures to model or manage
knowledge. To the best of our knowledge, the work by Cimiano et al.
\cite{Cimiano04} is the first study that investigated the possible
use of Ontology in FCA by first clustering text documents using an
ontology and then applying FCA. One recurrent problem in FCA is the
huge number of concepts that can be derived from a data set since it
may be exponential in the size of the context. How can we handle
this problem? Many techniques have been proposed \cite{Cimiano04} in
order to use or produce a taxonomy on attributes or objects to
control the size of the context and the corresponding concept
lattice. Another trend is to query pattern bases (e.g., rules and
concepts) in a similar way as querying databases \cite{MKQV09} in
order to display the patterns that are the most relevant to the
user.

Patterns are a concise and semantically rich representation of data
\cite{Bertino04}. These can be clusters, concepts, association
rules, decision trees, etc\dots. In this work we analyze some
possible ways to abstract (group) objects/attributes together to get
generalized patterns such as generalized itemsets and association
rules \cite{Srikant95}. The problem we address in this paper is the
use of taxonomies on attributes or objects to produce and manipulate
generalized patterns.

The rest of this contribution is organized as follows. In
Section~\ref{S:FCA} we introduce the basic notions of FCA.
Section~\ref{S:genpatterns} presents different ways to group
attributes/objects to produce generalized patterns. In
Section~\ref{S:visual} we discuss line diagrams of generalized
patterns while in Section~\ref{S:LattSize} the size of the
generalized concept set is compared to the size of the initial
(before generalization) concept set. Some experimental results are
shown in Section \ref{S:experiments}. Finally, existing work about
combining FCA with Ontology is briefly described in Section
\ref{S:relatedwork}.

 %Finally we discuss in Section~\ref{S:auto} how a taxonomy can be
% derived from the initial context, to produce generalized patterns.


==> Sect5+6.tex <==
\section{Controlling the size of generalized concepts}\label{S:LattSize}
We call a concept generalized if its intent or extent contains
generalized attributes or generalized objects.
\subsection{An $\exists$-generalization on attributes}
Let $(G,M,I)$ be a context and $(G,S,J)$ a context obtained from an
$\exists$-generalization on attributes, i.e the elements of $S$ are
groups of attributes from $M$. We set $S=\{m_s\mid s\in S\}$, with
$m_s\subseteq M$. Then an object $g\in G$ is in relation with a
generalized attribute $m_s$ if there is an attribute $m$ in $m_s$
such that $g\I m$.  To compare the size of the corresponding concept
lattices, we will define some correspondences. We assume that
$(m_s)_{s\in S}$ forms a partition of $M$. Then for each $m\in M$
there is a unique generalized attribute $m_s$ such that $m\in m_s$,
and $g\I m$ implies $g\J m_s$, for every $g\in G$.
 \[
\begin{array}{rcl}
\alpha\colon G & \to & \mathfrak{B}(G,S,J) \\
  g & \mapsto & \bar{{\gamma}}g:=(g\sp{\J\J},g\sp{\J})
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\beta \colon  M & \to & \mathfrak{B}(G,S,J) \\
 m & \mapsto & \bar{{\mu}}m_s:=(s\sp{\J},s\sp{\J\J}), \mbox{ where } m\in m_s
\end{array}
\]
The maps $\alpha$ and $\beta$ induce two order preserving maps
$\varphi$ and $\psi$ defined by
 \[
\begin{array}{rcl}
\varphi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigvee\{{\alpha}g\mid g\in A\}
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\psi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigwedge\{{\beta}m\mid m\in B\}
\end{array}
\]
If $\varphi$ or $\psi$ is surjective, then the generalized context
is of smaller cardinality. As we have seen on
Figure~\ref{fig:counterexplGen} these maps can be both not
surjective. Next we will examine some special cases. Obviously
$\varphi(A,B)\leq\psi(A,B)$, since $g\I m$ implies $g\J m_s$, and
$\bar{{\gamma}}g\leq\bar{{\mu}m_s}$.
\begin{description}
\item[Case 1] Every $m_s$ has a greatest element $1_s$. Then the context $(G,S,J)$ is a projection of $(G,M,I)$ on the set $M_S:=\{1_s\mid s\in S\}$ of greatest elements of $m_s$. Thus $\frak{B}(G,S,J)\cong\frak{B}(G,M_S,I\cap(G\times M_S))$ and is a sub-order of $\frak{B}(G,M,I)$. Hence $|\frak{B}(G,S,J)|=|\frak{B}(G,M_S,I\cap G\times M_S)|\leq|\frak{B}(G,M,I)|$.
\item[Case 2] The context $(G,M,I)$ is object reduced and the lattice $\frak{B}(G,M,I)$ distributive. Since $m_s^{\J}=\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$, then $m_s^{\J}$ is an extent of $(G,M,I)$. preuve.  Therefore, the grouping of attributes in $m_s$ does not produce a new concept.
\item[Case 3] The union $\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$. Then any grouping does not produce a new concept, then the number of concept cannot increase.
\item[Case 4] We do the grouping one after another. If the number of concept produce in one step is less than the number of concepts deleted, then smaller size.  See statistics.
\item[Case 5] The overall number of new concepts is less than the deleted. Then smaller size.
\end{description}
\subsection{A $\forall$-generalization on attributes}
Let $(G,S,J)$ be a context obtained from $(G,M,I)$ by a
$\forall$-generalization. In the context $(G,M\cup S, I\cup J)$,
each attribute concept ${\mu}m_s$ is reducible. In fact
$m_s^{\J}=\bigcap\{m^{\J}\mid m\in m_s\}=\bigcap\{m^{\I}\mid m\in
m_s\}$, and is an extent of $(G,M,I)$. Therefore
$|\frak{B}(G,S,J)|\leq|\frak{B}(G,M\cup S,I\cup
J)|=|\frak{B}(G,M,I)|$.
\section{Semi automatic generalization process}
To motivate this process we consider a data mining context
$(G,M,I)$, where $G$ is the set of transactions and $M$ the set of
items. With an $\exists$-generalization, some items that where non
frequent can become frequent. So, the idea is to start from the set
of items $M$, keep the frequent items from $M$, and put the non
frequent items in groups so that at least a certain percentage of
transactions contains at least one object from each group. This can
be done with the help of a computer program; it will propose some
groupings to the user for validation.

For a $\forall$-generalization, a choice can be some intents. i.e.
some concept intents are replaced by a single attribute.


For an $\alpha$-generalization, the idea is to replace the
fault-tolerant intent with a single attribute. Attention!

From a taxonomy $T$, we will choose a transversal $\mathcal{E}$ and
roll up to one or more levels, or roll down for one or more levels.


==> Section5+6.tex <==
\section{Controlling the size of generalized concepts}\label{S:LattSize}
We call a concept generalized if its intent or extent contains
generalized attributes or generalized objects.
\subsection{An $\exists$-generalization on attributes}
Let $(G,M,I)$ be a context and $(G,S,J)$ a context obtained from an
$\exists$-generalization on attributes, i.e the elements of $S$ are
groups of attributes from $M$. We set $S=\{m_s\mid s\in S\}$, with
$m_s\subseteq M$. Then an object $g\in G$ is in relation with a
generalized attribute $m_s$ if there is an attribute $m$ in $m_s$
such that $g\I m$.  To compare the size of the corresponding concept
lattices, we will define some correspondences. We assume that
$(m_s)_{s\in S}$ forms a partition of $M$. Then for each $m\in M$
there is a unique generalized attribute $m_s$ such that $m\in m_s$,
and $g\I m$ implies $g\J m_s$, for every $g\in G$.
 \[
\begin{array}{rcl}
\alpha\colon G & \to & \mathfrak{B}(G,S,J) \\
  g & \mapsto & \bar{{\gamma}}g:=(g\sp{\J\J},g\sp{\J})
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\beta \colon  M & \to & \mathfrak{B}(G,S,J) \\
 m & \mapsto & \bar{{\mu}}m_s:=(s\sp{\J},s\sp{\J\J}), \mbox{ where } m\in m_s
\end{array}
\]
The maps $\alpha$ and $\beta$ induce two order preserving maps
$\varphi$ and $\psi$ defined by
 \[
\begin{array}{rcl}
\varphi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigvee\{{\alpha}g\mid g\in A\}
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\psi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigwedge\{{\beta}m\mid m\in B\}
\end{array}
\]
If $\varphi$ or $\psi$ is surjective, then the generalized context
is of smaller cardinality. As we have seen on
Figure~\ref{fig:counterexplGen} these maps can be both not
surjective. Next we will examine some special cases. Obviously
$\varphi(A,B)\leq\psi(A,B)$, since $g\I m$ implies $g\J m_s$, and
$\bar{{\gamma}}g\leq\bar{{\mu}m_s}$.
\begin{description}
\item[Case 1] Every $m_s$ has a greatest element $1_s$. Then the context $(G,S,J)$ is a projection of $(G,M,I)$ on the set $M_S:=\{1_s\mid s\in S\}$ of greatest elements of $m_s$. Thus $\frak{B}(G,S,J)\cong\frak{B}(G,M_S,I\cap(G\times M_S))$ and is a sub-order of $\frak{B}(G,M,I)$. Hence $|\frak{B}(G,S,J)|=|\frak{B}(G,M_S,I\cap G\times M_S)|\leq|\frak{B}(G,M,I)|$.
\item[Case 2] The context $(G,M,I)$ is object reduced and the lattice $\frak{B}(G,M,I)$ distributive. Since $m_s^{\J}=\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$, then $m_s^{\J}$ is an extent of $(G,M,I)$. preuve.  Therefore, the grouping of attributes in $m_s$ does not produce a new concept.
\item[Case 3] The union $\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$. Then any grouping does not produce a new concept, then the number of concept cannot increase.
\item[Case 4] We do the grouping one after another. If the number of concept produce in one step is less than the number of concepts deleted, then smaller size.  See statistics.
\item[Case 5] The overall number of new concepts is less than the deleted. Then smaller size.
\end{description}
%{\bf Claim: Any grouping can increase only in 1 the number of concepts. }

% surjective iff %since %${\alpha}G$ is $\vee$-dense and ${\beta}M$ is
% $\wedge$-dense in $\mathfrak{B}(G,S,J)$. However $\varphi$ does
% not necessary preserve suprema.
% Note that
% We consider the  maps
% \[
% \begin{array}{rclcl}
% \phi & \colon & G & \to & \mathfrak{B}(G,S,J) \\
%  & & g & \mapsto & (g\sp{JJ},g\sp{J})
%  \end{array}\quad
%  \mbox{ and }\quad
%  \begin{array}{rclcl}
% \psi & \colon & M & \to & \mathfrak{B}(G,S,J) \\
%  & & m & \mapsto & (s\sp{J},s\sp{JJ}) \mbox{ with } m\in M_s.
%  \end{array}
%  \]
% Thus $\phi$ and $\psi$  induce an order preserving map (for example $\varphi:(A,B)\mapsto\bigvee\{{\phi}g\mid g\in A\}$)  from $\mathfrak{B}(G,M,I)$ to $\mathfrak{B}(G,S,J)$ since $(g\sp{JJ},g\sp{J})={\phi}g\leq{\psi}m=(s\sp{J},s\sp{JJ})$
%  (see~\cite[Prop.33]{Ganter+1999}).
% $\wedge$-dense in $\mathfrak{B}(G,S,J)$. However $\varphi$ does
% not necessary preserve suprema.
% Note that
%   for $A\subseteq G$ we have
%  \[A\sp{II}:=\{g\in G\mid A\subseteq m'\implies g\in m'\}\] and
%  \[A\sp{JJ}:=\{g\in G\mid A\subseteq {\bigcup\sb{m\in M_s}}m' \implies g\in {\bigcup\sb{m\in M_s}}m' \}.\]
% Therefore $A\subseteq A\sp{II}\subseteq A\sp{JJ}$ and
% $A\sp{JJ}=(A\sp{II})\sp{JJ}$. Moreover
% \[\bigvee\sb{g\in A}(g\sp{JJ},g\sp{J})=(A\sp{JJ},A\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% %\[\bigvee\sb{g\in A\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% Thus for a concept $(U,U\sp{J})$ of $\mathfrak{B}(G,S,J)$, the
% pair $(U\sp{II},U\sp{I})$ is a concept of $\mathfrak{B}(G,M,I)$
% and
% \[\varphi(U\sp{II},U\sp{I})= \bigvee\sb{g\in U\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% (U\sp{II})\sp{JJ}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% U\sp{JJ}}(g\sp{JJ},g\sp{J}) =(U,V).\]

\subsection{A $\forall$-generalization on attributes}
Let $(G,S,J)$ be a context obtained from $(G,M,I)$ by a
$\forall$-generalization. In the context $(G,M\cup S, I\cup J)$,
each attribute concept ${\mu}m_s$ is reducible. In fact
$m_s^{\J}=\bigcap\{m^{\J}\mid m\in m_s\}=\bigcap\{m^{\I}\mid m\in
m_s\}$, and is an extent of $(G,M,I)$. Therefore
$|\frak{B}(G,S,J)|\leq|\frak{B}(G,M\cup S,I\cup
J)|=|\frak{B}(G,M,I)|$.

\section{Semi automatic generalization process}
To motivate this process we consider a data mining context
$(G,M,I)$, where $G$ is the set of transactions and $M$ the set of
items. With an $\exists$-generalization, some items that where non
frequent can become frequent. So, the idea is to start from the set
of items $M$, keep the frequent items from $M$, and put the non
frequent items in groups so that at least a certain percentage of
transactions contains at least one object from each group. This can
be done with the help of a computer program; it will propose some
groupings to the user for validation.

For a $\forall$-generalization, a choice can be some intents. i.e.
some concept intents are replaced by a single attribute.


For an $\alpha$-generalization, the idea is to replace the
fault-tolerant intent with a single attribute. Attention!

From a taxonomy $T$, we will choose a transversal $\mathcal{E}$ and
roll up to one or more levels, or roll down for one or more levels.


==> fcaintro2.tex <==
\section{Ontologies and taxonomies}



==> genattrib.tex <==
\def\J{\mathop{\mbox{\rm J}}}
\def\imp{\mathop{\mbox{\rm Imp}}}
\def\ext{\mathop{\mbox{\rm ext}}}
\def\int{\mathop{\mbox{\rm int}}}
\section{Generalized Patterns}
The objective here is to exploit generalization hierarchies attached
to properties to get a lattice with more abstract concepts.
Producing generalized patterns from concept lattices when a taxonomy
on attributes is provided can be done in different ways with
distinct performance costs that depend on the peculiarities of the
input (e.g., size, density) and the operations used. One way
consists to use context apposition \cite{Ganter+1999} to conduct the
assembly (join) of the initial lattice of non generalized attributes
(e.g., destinations of airline companies) with the lattice
corresponding to the taxonomy of attributes (e.g., city, country,
continent), and then perform a projection of the resulting lattice
on the generalized attributes (e.g., country) only.

In the following we formalize the way generalized patterns are
produced. Let $\mathbb{K}:=(G,M,I)$ be a context. The attributes of
$\mathbb{K}$ can be grouped together to form another set of
attributes, namely $S$, to get a context where the attributes are
more general than in $\mathbb{K}$. For the Star Alliance example,
each member is flying to an airport located in a city. Cities are
generalized to countries and sometimes to regions or continents.
Formally, $S$ can be seen as an index set such that $\{M_s\mid s\in
S\}$ covers $M$. The context $(G,M,I)$ is then replaced with a
context $(G,S,J)$ as in the scaling process.
There are mainly three ways to express the binary relation $J$ between the objects of $G$ and the (generalized) attributes of $S$:
%There are mainly three cases:
\begin{itemize}
\item[$(\exists)$] $g\J s:\iff \exists m\in s,\, g\I m$. Consider an information table describing companies and their branches in North America. We first set up a context whose objects are companies and whose attributes are the cities where these companies have or may have branches. If there are too many cities, we can decide to group them into provinces (in Canada) or states (in USA) to reduce the number of attributes. Then, the (new) set of attributes is now a set $S$ whose elements are states and provinces. It is quite natural to say that a company $g$ has a branch in a province/state $s$ if $g$ has a branch in a city $m$ which belongs to the province/state $s$. Formally, $g$ has attribute $s$ iff there is $m\in s$ such that $g$ has attribute $m$. %The symbol $\in$ can be extended to mean not only \emph{is a member of a set} but also \emph{is an instance of} (\emph{e.g.}, Jean is a university President) or \emph{is a kind of} (\emph{e.g.}, a faculty member is a university employee).
\item[$(\forall)$] $g\J s:\iff \forall m\in s,\, g\I m$. Consider an information system about Ph.D. students and the components of the comprehensive doctoral exam. Assume that components are: the written part, the oral part, and the thesis proposal,  and that a student succeeds in his exam if he succeeds in the three components of the exam. The objects of the context are Ph.D. students and the attributes are the different exams taken by students. If we group together the different components, for example
\[CE.written, CE.oral, CE.proposal\mapsto CE.exam,\]
then it becomes natural to say that a student $g$ succeeds in his comprehensive exam $CE.exam$ if he succeeds in {\it all} the exam parts of $CE$. i.e $g$ has attribute $CE.exam$ if for all $m$ in $CE.exam$, $g$ has attribute $m$.
\item[$(\alpha\%)$] $g\J s:\iff \frac{|\{m\in s\ \mid\ g\I m\}|}{|s|}\geq\alpha_s$ where $\alpha_s$ is a threshold set by the user for the generalized attribute $s$. This case generalizes the $(\exists)$-case (take $\alpha=\frac{1}{|M|}$) and the $(\forall)$-case (take $\alpha=1$). To illustrate this case, let us consider a context describing different specializations in a given Master degree program. For each program there is a set of mandatory courses and a set of optional ones. Moreover, there is a predefined number of courses that a student should succeed to get a degree in a given specialization. Assume that to get a Master in Computer Science with a specialization in ``computational logic'' (CL), a student must have seven courses from a set $s_1$ of mandatory courses and three courses from a set $s_2$ of optional ones. Then we can introduce two generalized attributes $s_1$ and $s_2$ so that a student $g$ succeeds in the group $s_1$ if he succeeds in at least seven courses from $s_1$, and succeeds in $s_2$ if he succeeds in at least three courses from $s_2$. So, for $\alpha_{s_1}:=\frac{7}{|s_1|}$ and $\alpha_{s_2}:=\frac{3}{|s_2|}$, we have
\[g\J s_i\iff\frac{|\{m\in s_i\ \mid\ g\I m\}|}{|s_i|}\geq\alpha_{s_i}, \ 1\leq i\leq 2.\]
\end{itemize}
 Attribute generalization reduces the number of attributes. One may therefore expect a reduction of
 the number of concepts (i.e., $|\frak{B}(G,S,J)|\leq |\frak{B}(G,M,I)|$).
 Unfortunately, this is not always the case, as we can see from example in Figure ~\ref{fig:counterexplGen} below.
 Therefore, it is interesting to investigate under which condition generalizing patterns reduces the
 size of the initial lattice (see Section~\ref{S:LattSize}).
 Moreover, finding the connections between the implications and more generally association rules of the generalized context and the initial one is also
 an important open problem to be considered later.
 %(see Section~\ref{S:genImp}).

\begin{figure}
\begin{minipage}{.50\textwidth}
\begin{cxt}
\cxtName{$\KK$}%
\att{$m_1$}%
\att{$m_2$}%
\att{$m_3$}%
\att{$m_4$}%
\att{$m_5$}%
\att{$m_6$}%
\obj{..xxxx}{$g_1$}%
\obj{.x.xx.}{$g_2$}%
\obj{x.x.x.}{$g_3$}%
\obj{xxxxxx}{$g_4$}%
\obj{....x.}{$g_5$}%
\end{cxt}
\end{minipage}
\quad
\begin{minipage}{.40\textwidth}
\parbox{5cm}{\includegraphics[scale=.40]{SmallContext.png}}

% \begin{diagram}{80}{90}
% %\CircleSize{3}
% \Node{1}{40}{20}
% \Node{2}{20}{40}
% \Node{3}{40}{40}
% \Node{4}{60}{40}
% \Node{5}{20}{60}
% \Node{6}{60}{60}
% \Node{7}{40}{80}

% \Edge{1}{2} \Edge{1}{3} \Edge{1}{4}
% \Edge{2}{5} \Edge{3}{5} \Edge{3}{6}
% \Edge{4}{6} \Edge{5}{7} \Edge{6}{7}

% \leftAttbox{2}{2}{2}{$m_1$} \rightAttbox{4}{2}{2}{$m_2$}
% \leftAttbox{5}{2}{2}{$m_3$} \rightAttbox{6}{2}{2}{$m_4$}
% \rightAttbox{3}{0}{4}{$m_6$} \rightAttbox{7}{2}{2}{$m_5$}

% \leftObjbox{2}{2}{2}{$g_3$} \leftObjbox{3}{2}{2}{$g_1$}
% \rightObjbox{4}{2}{2}{$g_2$} \leftObjbox{1}{2}{2}{$g_4$}
% \leftObjbox{7}{0}{4}{$g_5$}
% \end{diagram}
\end{minipage}
\caption{A small context and its line diagram. The $g_i$'s are transactions and the $m_i$'s items.}
\label{fig:smallcxt}
\end{figure}

\begin{figure}
\begin{minipage}{.50\textwidth}
\begin{cxt}
\cxtName{$\KK_{\text{gen}}$}
\att{$m_{12}$}%
\att{$m_3$}%
\att{$m_4$}%
\att{$m_5$}%
\att{$m_6$}%

\obj{.xxxx}{$g_1$}%
\obj{x.xx.}{$g_2$}%
\obj{xx.x.}{$g_3$}%
\obj{xxxxx}{$g_4$}%
\obj{...x.}{$g_5$}%
\end{cxt}
\end{minipage}
\quad
\begin{minipage}{.40\textwidth}
\parbox{5cm}{\includegraphics[scale=.40]{SmallContextG.png}}

% \begin{diagram}{80}{90}
% %\CircleSize{3}
% \Node{1}{40}{20}
% \Node{2}{20}{40}
% \Node{3}{40}{40}
% \Node{4}{60}{40}
% \Node{5}{20}{60}
% \Node{6}{60}{60}
% \Node{7}{40}{80}
% \Node{8}{40}{60}


% \Edge{1}{2} \Edge{1}{3} \Edge{1}{4}
% \Edge{2}{5} \Edge{3}{5} \Edge{3}{6}
% \Edge{4}{6} \Edge{5}{7} \Edge{6}{7}
% \Edge{2}{8} \Edge{4}{8} \Edge{7}{8}


% %\leftAttbox{2}{2}{2}{$m_1$} \rightAttbox{4}{2}{2}{$m_2$}
% \rightAttbox{8}{2}{2}{$m_{12}$}

% \leftAttbox{5}{2}{2}{$m_3$} \rightAttbox{6}{2}{2}{$m_4$}
% \rightAttbox{3}{0}{4}{$m_6$} \rightAttbox{7}{2}{2}{$m_5$}

% \leftObjbox{2}{2}{2}{$g_3$} \leftObjbox{3}{2}{2}{$g_1$}
% \rightObjbox{4}{2}{2}{$g_2$} \leftObjbox{1}{2}{2}{$g_4$}
% \leftObjbox{7}{0}{4}{$g_5$}
% \end{diagram}
\end{minipage}
\caption{The context $\KK_{\text{gen}}$ is obtained from the context
$\KK$ in Figure~\ref{fig:smallcxt} by putting together the
attributes $m_1$ and $m_2$ to get $m_{12}$ as an
$\exists$-generalization. The number of concepts in
$\KK_{\text{gen}}$ has increased.
$|\frak{B}(\KK)|=7<8=|\frak{B}(\KK_{\text{gen}})|$.}
\label{fig:counterexplGen}
\end{figure}

The following context can be seen as an apposition of two
sub-contexts $\KK_1:=(G,S_1,J_1)$ and $\KK_2:=(G,S_2,J_2)$ where
$S_1=\{A, B, C, D\}$ is the set of attributes obtained from an
$\exists$-generalization and  $S_2=\{S, T, U, V\}$ is the set of
attributes obtained from a $\forall$-generalization of original
attributes. More specifically, A= e ou g, B: b ou c, C: a ou d, D: f
ou h. S: e et g, T: b et c,  U: a et d, V: f et h.


\begin{figure}[htbp]
\begin{minipage}{.30\textwidth}
\begin{cxt}
\cxtName{$\KK_\exists$}%
\att{A}%
\att{B}%
\att{C}%
\att{D}%
% \att{E}%
% \att{F}%
% \att{S}%
% \att{T}%
% \att{U}%
% \att{V}%
\obj{x.x.}{1}%
\obj{x.xx}{2}%
\obj{xxxx}{3}%
\obj{xx.x}{4}%
\obj{.xx.}{5}%
\obj{.xx.}{6}%
\obj{xx..}{7}%
\obj{xxx.}{8}%
\end{cxt}
\end{minipage}
\parbox{5cm}{\includegraphics[scale=.40]{LatticeABCD.png}}

\begin{minipage}{.30\textwidth}
\begin{cxt}
\cxtName{$\KK_\forall$}%
% \att{A}%
% \att{B}%
% \att{C}%
% \att{D}%
% \att{E}%
% \att{F}%
\att{S}%
\att{T}%
\att{U}%
\att{V}%
\obj{x...}{1}%
\obj{...x}{2}%
\obj{x..x}{3}%
\obj{..x.}{4}%
\obj{.xx.}{5}%
\obj{.x..}{6}%
\obj{.x..}{7}%
\obj{.x..}{8}%
\end{cxt}
\end{minipage}
\hspace{0.1cm}
\parbox{4.5cm}{\includegraphics[scale=.40]{LatticeSTUV.png}
}
\caption{\small Generalized concepts using $\exists$ case (left) and
$\forall$ case (right).} \label{fig:GenLattice}
\end{figure}



 A similar reasoning can be conducted with objects (rather than attributes) to replace some (or all) of them with generalized objects. A typical situation would be that of two or more star alliance members (or companies in general) amalgamating. They can keep all their destinations (an $\exists$-generalization) or keep only their common destinations (a $\forall$-generalization), or keep just some of their destinations with respect to some agreement (similar to an $\alpha$-generalization). We are aware that the two companies can also abandon some of their destinations and/or open new ones after amalgamating. But we do not consider formalizing this case in this paper.  An $\alpha$-generalization has been applied on text as pre-treatment to get clusters\cite{Hotho03}. Citer travaux de Soldano et Ventos.

In order to reduce the size of the data to be analyze, both technics can apply: generalizing attributes and then objects or vice-versa or simultaneously. This can be seen as a pre-treatment on the data in order to reduce and then have a better overview on the data to be analyzed. Done simultaneously, combining the generalizations on attributes and on objects will give a kind of {\em hypercontext} (similar to hypergraphs\cite{}), since the objects are subsets of $G$ and attributes subsets of $M$. Let $\cal{A}$ be a group of objects and $\cal{B}$ be a group of attributes. The relation $\J$ will can be defined using one of the following cases below:
\begin{enumerate}
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff some objects from the group $\cal{E}$ are in relation $\I$ with some attributes in the group $\cal{B}$ , i.e. $\cal{A}\J\cal{B}$ iff $\exists a\in\cal{A}$, $\exists b\in\cal{B}$ such that $a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff every object in the group $\cal{A}$ is in relation $\I$ with every attribute in the group $\cal{B}$, i.e. $\cal{A}\J\cal{B}$ iff $\forall a\in\cal{A}$, $\forall b\in\cal{B}\  a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff every object in the group $\cal{A}$ has at least one attribute from the group $\cal{B}$, i.e. $\cal{A}\J\cal{B}$ iff $\forall a\in\cal{A}$, $\exists b\in\cal{B}$ such that $a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff there is an attribute in the group $\cal{B}$ that belongs to all objects of the group $\cal{A}$, i.e. $\cal{A}\J\cal{B}$ iff $\exists b\in\cal{B}$ such that $\forall a\in\cal{A}$  $a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff every property in the group $\cal{B}$ is satisfied by at least one object of the group $\cal{A}$, i.e. $\cal{A}\J\cal{B}$ iff $\forall b\in\cal{B}$, $\exists a\in\cal{A}$ such that $a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ iff there is an object in the group $\cal{A}$ that has all the attributes in the group $\cal{B}$; i.e.  $\cal{A}\J\cal{B}$ iff $\exists a\in\cal{A}$ such that  $\forall b\in\cal{B}\ a\I b$.
\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ if at least $\alpha_{\cal{A}}\%$ of objects in the group $\cal{A}$ have each at least $\beta_{\cal{B}}\%$ attributes of the attributes in the group $\cal{B}$;
\[i.e.\qquad \cal{A}\J\cal{B} :\iff \frac{\left|a\in\cal{A}\mid \frac{|\{b\in\cal{B}\mid a\I b\}|}{|\cal{B}|}\geq \beta_{\cal{B}} \right|}{|\cal{A}|}\geq\alpha_\cal{A}\]
This generalizes the case $1.$ (take $\alpha_{\cal{A}}:=\frac{1}{|G|}$ and $\beta_{\cal{B}}:=\frac{1}{|M|}$ for all $\cal{A}$ and $\cal{B}$), the case $2.$ (take $\alpha_{\cal{A}}:=1$ and $\beta_{\cal{B}}:=1$ for all $\cal{A}$ and $\cal{B}$), the case $3.$ (take $\alpha_{\cal{A}}:=1$ and $\beta_{\cal{B}}:=\frac{1}{|M|}$ for all $\cal{A}$ and $\cal{B}$) and the case $5.$ (take $\alpha_{\cal{A}}:=\frac{1}{|G|}$ and $\beta_{\cal{B}}:=1$ for all $\cal{A}$ and $\cal{B}$). Note that cases 4 and 6 cannot be captured by this case.

\item A generalized object $\cal{A}$ is in relation $\J$ with a generalized attribute $\cal{B}$ if at least $\beta_{\cal{B}}\%$ of attributes in the group $\cal{B}$ belong altogether to at least $\alpha_{\cal{A}}\%$ of objects the objects in the group $\cal{A}$;
\[i.e.\qquad \cal{A}\J\cal{B} :\iff \frac{\left|\left\{b\in\cal{B}\mid
\frac{|\{a\in\cal{A}\mid a\I b\}|}{|\cal{A}|}\geq \alpha_{\cal{A}}\right\} \right|}{|\cal{B}|}\geq\beta_\cal{B}\]
This generalizes the case $1.$ (take $\alpha_{\cal{A}}:=\frac{1}{|G|}$ and $\beta_{\cal{B}}:=\frac{1}{|M|}$ for all $\cal{A}$ and $\cal{B}$), the case $2.$ (take $\alpha_{\cal{A}}:=1$ and $\beta_{\cal{B}}:=1$ for all $\cal{A}$ and $\cal{B}$), the case $3.$ (take $\alpha_{\cal{A}}:=1$ and $\beta_{\cal{B}}:=\frac{1}{|M|}$ for all $\cal{A}$ and $\cal{B}$) and the case $5.$ (take $\alpha_{\cal{A}}:=\frac{1}{|G|}$ and $\beta_{\cal{B}}:=1$ for all $\cal{A}$ and $\cal{B}$). Note that cases 4 and 6 cannot be captured by this case.

\end{enumerate}
We are going to see in the next section its impact on the size of concepts and rules extracted.
\section{Visualizing generalized patterns on line diagrams}
\subsection{Visualizing}
Let $(G,M,I)$ be a formal context and $(G,S,J)$ a context obtained from $(G,M,I)$ via a generalization on attributes. The usual reflex is to directly construct a line diagram of $(G,S,J)$. Then we get the concepts with generalized attributes. However, we have on mean, after getting $(G,S,J)$ and constructing a line diagram for $\frak{B}(G,S,J)$, to refine further back on the attributes in $M$ or to recover the operation we made on $(G,M,I)$.

Now if we have enough space, then we can keep the attributes in $M$ and the generalized attributes altogether. This is done using an apposition of $(G,M,I)$ and $(G,S,J)$ to get $(G,M\cup S,I\cup J)$. A nested line diagram  can be used to display the resulting lattice, with $(G,S,J)$ as first level and $(G,M,I)$ as second level; i.e. we construct a line diagram for $\frak{B}(G,S,J)$ with nodes large enough to contain copies of a line diagram of $\frak{B}(G,M,I)$.

The generalized attributes can also be visualized by conducting a projection on generalized attributes,  and keeping track of the effects of the projections; i.e, we display the projection of the concept lattice $\frak{B}(G,M\cup S,I\cup J)$ on $S$ by marking the equivalence classes on $\frak{B}(G,M\cup S, I\cup J)$.
\subsection{Are generalized attributes really generalizations?}
Let us have a close look at the concept lattice $\frak{B}(G,M\cup S, I\cup J)$. Recall that a concept $\frak{u}$ is more general than a concept $\frak{v}$, if $\frak{u}$ contains more objects than $\frak{v}$. That is $\frak{v}\leq\frak{u}$, or $\ext(\frak{v})\subseteq\ext(\frak{u})$, or $\int(\frak{u})\subseteq\int(\frak{v})$.  We also say that $\frak{u}$ is a generalization of $\frak{v}$, and $\frak{v}$ a specialization of $\frak{u}$. For two attribute $a$ and $b$ in $M\cup S$, we should normally say that $a$ is a generalization of $b$ or $b$ is a specialization of $a$ whenever ${\mu}a$ is a generalization of ${\mu}b$. Now let us have a close look at the generalization on attributes above.

In the $\exists$-case, an object $g\in G$ is in relation with an attribute $m_s$ iff there is $m\in m_s$ such that $g\I m$. Thus  $m_s'=\bigcup\{m'\mid m\in m_s\}$ and ${\mu}m_s=\bigvee\{{\mu}m\mid m\in m_s\}$. Therefore every generalized attribute $m_s$ satisfies ${\mu}m_s\geq{\mu}m$ for all $m\in m_s$, and deserves the name of a {\em generalization} of the attributes $m$'s, $m\in m_s$.

In the $\forall$-case, an object $g\in G$ is in relation with an attribute $m_s$ iff $g\I m$ for all $m\in m_s$. Thus  $m_s'=\bigcap\{m'\mid m\in m_s\}$ and ${\mu}m_s=\bigwedge\{{\mu}m\mid m\in m_s\}$. Therefore every generalized attribute $m_s$ satisfies ${\mu}m_s\leq{\mu}m$ for all $m\in m_s$, and should normally be called a {\em specialization} of the attributes $m$'s, $m\in m_s$.

In the $\alpha$-case, $\frac{1}{|M|}<\alpha<1$, an object $g\in G$ is in relation with an attribute $m_s$ iff $\alpha\leq\frac{|\{m\in m_s\mid g\I m\}|}{|m_s|}$. The following situations can happen:
\begin{itemize}
\item there is a generalized attribute $m_s\in S$ with at least one attribute $m\in m_s$ such that $g{\not\I}m$ and $g\J m_s$; hence ${\mu}m\nleq{\mu}m_s$ in $\frak{B}(G,M\cup S, I\cup J)$; i.e  ${\mu}m_s$ is not a {\em generalization} of ${\mu}m$, and by then not a {\em generalization} of the ${\mu}m$'s, $m\in m_s$ though it is so called.
\item there is a generalized attribute $m_s\in S$ with at least one attribute $m\in m_s$ such that $g\I m$ and $g{\not\J}m_s$;  hence ${\mu}m_s\nleq{\mu}m$ in $\frak{B}(G,M\cup S, I\cup J)$; i.e  ${\mu}m_s$ is not a {\em specialization} of ${\mu}m$, and by then not a {\em specialization} of the ${\mu}m$'s, $m\in m_s$.
\end{itemize}
Therefore there might exist a generalized attributes $m_s$ that is neither a {\em generalization} of the $m$'s nor a specialization of the $m$'s. Thus we should better call the $\alpha$-case an \neu{attribute approximation}, the $\forall$-case a \neu{specialization} and only the $\exists$-case a \neu{generalization}.
\section{Controlling the size of generalized concepts}\label{S:LattSize}
We call a concept generalized if its intent or extent contains generalized attributes or generalized objects.
\subsection{An $\exists$-generalization on attributes}
Let $(G,M,I)$ be a context and $(G,S,J)$ a context obtained from an $\exists$-generalization on attributes, i.e the elements of $S$ are groups of attributes from $M$. We set $S=\{m_s\mid s\in S\}$, with $m_s\subseteq M$. Then an object $g\in G$ is in relation with a generalized attribute $m_s$ if there is an attribute $m$ in $m_s$ such that $g\I m$.  To compare the size of the corresponding concept lattices, we will define some correspondences. We assume that $(m_s)_{s\in S}$ forms a partition of $M$. Then for each $m\in M$ there is a unique generalized attribute $m_s$ such that $m\in m_s$, and $g\I m$ implies $g\J m_s$, for every $g\in G$.
 \[
\begin{array}{rcl}
\alpha\colon G & \to & \mathfrak{B}(G,S,J) \\
  g & \mapsto & \bar{{\gamma}}g:=(g\sp{\J\J},g\sp{\J})
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\beta \colon  M & \to & \mathfrak{B}(G,S,J) \\
 m & \mapsto & \bar{{\mu}}m_s:=(s\sp{\J},s\sp{\J\J}), \mbox{ where } m\in m_s
\end{array}
\]
The maps $\alpha$ and $\beta$ induce two order preserving maps $\varphi$ and $\psi$ defined by
 \[
\begin{array}{rcl}
\varphi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigvee\{{\alpha}g\mid g\in A\}
\end{array}\quad
\mbox{ and }\quad
\begin{array}{rcl}
\psi:\mathfrak{B}(G,M,I) & \to &\mathfrak{B}(G,S,J)\\
 (A,B) &\mapsto &\bigwedge\{{\beta}m\mid m\in B\}
\end{array}
\]
If $\varphi$ or $\psi$ is surjective, then the generalized context is of smaller cardinality. As we have seen on Figure~\ref{fig:counterexplGen} these maps can be both not surjective. Next we will examine some special cases. Obviously $\varphi(A,B)\leq\psi(A,B)$, since $g\I m$ implies $g\J m_s$, and $\bar{{\gamma}}g\leq\bar{{\mu}m_s}$.
\begin{description}
\item[Case 1] Every $m_s$ has a greatest element $1_s$. Then the context $(G,S,J)$ is a projection of $(G,M,I)$ on the set $M_S:=\{1_s\mid s\in S\}$ of greatest elements of $m_s$. Thus $\frak{B}(G,S,J)\cong\frak{B}(G,M_S,I\cap(G\times M_S))$ and is a sub-order of $\frak{B}(G,M,I)$. Hence $|\frak{B}(G,S,J)|=|\frak{B}(G,M_S,I\cap G\times M_S)|\leq|\frak{B}(G,M,I)|$.
\item[Case 2] The context $(G,M,I)$ is object reduced and the lattice $\frak{B}(G,M,I)$ distributive. Since $m_s^{\J}=\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$, then $m_s^{\J}$ is an extent of $(G,M,I)$. preuve.  Therefore, the grouping of attributes in $m_s$ does not produce a new concept.
\item[Case 3] The union $\bigcup\{m^{\I}\mid m\in m_s\}$ for any $m_s\in S$. Then any grouping does not produce a new concept, then the number of concept cannot increase.
\item[Case 4] We do the grouping one after another. If the number of concept produce in one step is less than the number of concepts deleted, then smaller size.  See statistics.
\item[Case 5] The overall number of new concepts is less than the deleted. Then smaller size.
\end{description}
%{\bf Claim: Any grouping can increase only in 1 the number of concepts. }

% surjective iff %since %${\alpha}G$ is $\vee$-dense and ${\beta}M$ is
% $\wedge$-dense in $\mathfrak{B}(G,S,J)$. However $\varphi$ does
% not necessary preserve suprema.
% Note that
% We consider the  maps
% \[
% \begin{array}{rclcl}
% \phi & \colon & G & \to & \mathfrak{B}(G,S,J) \\
%  & & g & \mapsto & (g\sp{JJ},g\sp{J})
%  \end{array}\quad
%  \mbox{ and }\quad
%  \begin{array}{rclcl}
% \psi & \colon & M & \to & \mathfrak{B}(G,S,J) \\
%  & & m & \mapsto & (s\sp{J},s\sp{JJ}) \mbox{ with } m\in M_s.
%  \end{array}
%  \]
% Thus $\phi$ and $\psi$  induce an order preserving map (for example $\varphi:(A,B)\mapsto\bigvee\{{\phi}g\mid g\in A\}$)  from $\mathfrak{B}(G,M,I)$ to $\mathfrak{B}(G,S,J)$ since $(g\sp{JJ},g\sp{J})={\phi}g\leq{\psi}m=(s\sp{J},s\sp{JJ})$
%  (see~\cite[Prop.33]{Ganter+1999}).
% $\wedge$-dense in $\mathfrak{B}(G,S,J)$. However $\varphi$ does
% not necessary preserve suprema.
% Note that
%   for $A\subseteq G$ we have
%  \[A\sp{II}:=\{g\in G\mid A\subseteq m'\implies g\in m'\}\] and
%  \[A\sp{JJ}:=\{g\in G\mid A\subseteq {\bigcup\sb{m\in M_s}}m' \implies g\in {\bigcup\sb{m\in M_s}}m' \}.\]
% Therefore $A\subseteq A\sp{II}\subseteq A\sp{JJ}$ and
% $A\sp{JJ}=(A\sp{II})\sp{JJ}$. Moreover
% \[\bigvee\sb{g\in A}(g\sp{JJ},g\sp{J})=(A\sp{JJ},A\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% %\[\bigvee\sb{g\in A\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% Thus for a concept $(U,U\sp{J})$ of $\mathfrak{B}(G,S,J)$, the
% pair $(U\sp{II},U\sp{I})$ is a concept of $\mathfrak{B}(G,M,I)$
% and
% \[\varphi(U\sp{II},U\sp{I})= \bigvee\sb{g\in U\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% (U\sp{II})\sp{JJ}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% U\sp{JJ}}(g\sp{JJ},g\sp{J}) =(U,V).\]

\subsection{A $\forall$-generalization on attributes}
Let $(G,S,J)$ be a context obtained from $(G,M,I)$ by a
$\forall$-generalization. In the context $(G,M\cup S, I\cup J)$,
each attribute concept ${\mu}m_s$ is reducible. In fact
$m_s^{\J}=\bigcap\{m^{\J}\mid m\in m_s\}=\bigcap\{m^{\I}\mid m\in
m_s\}$, and is an extent of $(G,M,I)$. Therefore
$|\frak{B}(G,S,J)|\leq|\frak{B}(G,M\cup S,I\cup
J)|=|\frak{B}(G,M,I)|$.

\section{Semi automatic generalization process}
To motivate this process we consider a data mining context
$(G,M,I)$, where $G$ is the set of transactions and $M$ the set of
items. With an $\exists$-generalization, some items that where non
frequent can become frequent. So, the idea is to start from the set
of items $M$, keep the frequent items from $M$, and put the non
frequent items in groups so that at least a certain percentage of
transactions contains at least one object from each group. This can
be done with the help of a computer program; it will propose some
groupings to the user for validation.

For a $\forall$-generalization, a choice can be some intents. i.e. some concept intents are replaced by a single attribute.


For an $\alpha$-generalization, the idea is to replace the fault-tolerant intent with a single attribute. Attention!

From a taxonomy $T$, we will choose a transversal $\mathcal{E}$ and roll up to one or more levels, or roll down for one or more levels.


==> smallsizegen.tex <==
 Of course the size of $(G,S,J)$ is smaller than that of $(G,M,I)$. We also expect the size $\frak{B}(G,S,J)$ to be smaller that that of $\frak{B}(G,S,J)$. Unfortunately this is not always the case, as we can learn from example XXX below. Therefore it is interesting to investigate under which condition generalizing pattern reduces the size of the initial lattice. 
We consider the  maps
\[
\begin{array}{rclcl}
\phi & \colon & G & \to & \mathfrak{B}(G,S,J) \\
 & & g & \mapsto & (g\sp{JJ},g\sp{J})
 \end{array}\quad
 \mbox{ and }\quad
 \begin{array}{rclcl}
\psi & \colon & M & \to & \mathfrak{B}(G,S,J) \\
 & & m & \mapsto & (s\sp{J},s\sp{JJ}) \mbox{ with } m\in M_s.
 \end{array}
 \]
In the $(\exists)$-case we have $\forall m\in M_s,\ gIm\implies gJs$. Thus $\phi$ and $\psi$  induce an order preserving map (for example $\varphi:(A,B)\mapsto\bigvee\{{\phi}g\mid g\in A\}$)  from $\mathfrak{B}(G,M,I)$ to $\mathfrak{B}(G,S,J)$ since $(g\sp{JJ},g\sp{J})={\phi}g\leq{\psi}m=(s\sp{J},s\sp{JJ})$
 (see~\cite[Prop.33]{Ganter+1999}). If $\varphi$ is surjective then the generalized context is of small cardinality. %${\alpha}G$ is $\vee$-dense and ${\beta}M$ is
% $\wedge$-dense in $\mathfrak{B}(G,S,J)$. However $\varphi$ does
% not necessary preserve suprema.
% Note that
%   for $A\subseteq G$ we have
%  \[A\sp{II}:=\{g\in G\mid A\subseteq m'\implies g\in m'\}\] and
%  \[A\sp{JJ}:=\{g\in G\mid A\subseteq {\bigcup\sb{m\in M_s}}m' \implies g\in {\bigcup\sb{m\in M_s}}m' \}.\]
% Therefore $A\subseteq A\sp{II}\subseteq A\sp{JJ}$ and
% $A\sp{JJ}=(A\sp{II})\sp{JJ}$. Moreover
% \[\bigvee\sb{g\in A}(g\sp{JJ},g\sp{J})=(A\sp{JJ},A\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% %\[\bigvee\sb{g\in A\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in A\sp{JJ}}(g\sp{JJ},g\sp{J}).\]
% Thus for a concept $(U,U\sp{J})$ of $\mathfrak{B}(G,S,J)$, the
% pair $(U\sp{II},U\sp{I})$ is a concept of $\mathfrak{B}(G,M,I)$
% and
% \[\varphi(U\sp{II},U\sp{I})= \bigvee\sb{g\in U\sp{II}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% (U\sp{II})\sp{JJ}}(g\sp{JJ},g\sp{J})=\bigvee\sb{g\in
% U\sp{JJ}}(g\sp{JJ},g\sp{J}) =(U,V).\]
%  Thus the size of $\mathfrak{B}(G,S,J)$ is smaller than that of
%  $\mathfrak{B}(G,M,I)$.

